TangibleNet: Synchronous Network Data Storytelling through Tangible Interactions in Augmented Reality

Synchronous data-driven storytelling with network visualizations presents significant challenges due to the complexity of real-time manipulation of network components. While existing research addresses asynchronous scenarios, there is a lack of effective tools for live presentations. To address this gap, we developed TangibleNet, a projector-based AR prototype that allows presenters to interact with node-link diagrams using double-sided magnets during live presentations. The design process was informed by interviews with professionals experienced in synchronous data storytelling and workshops with 14 HCI/VIS researchers. Insights from the interviews helped identify key design considerations for integrating physical objects as interactive tools in presentation contexts. The workshops contributed to the development of a design space mapping user actions to interaction commands for node-link diagrams. Evaluation with 12 participants confirmed that TangibleNet supports intuitive interactions and enhances presenter autonomy, demonstrating its effectiveness for synchronous network-based data storytelling.

==> main <==
%%% -*-BibTeX-*-
%%% Do NOT edit. File created by BibTeX with style
%%% ACM-Reference-Format-Journals [18-Jan-2012].

\begin{thebibliography}{73}

%%% ====================================================================
%%% NOTE TO THE USER: you can override these defaults by providing
%%% customized versions of any of these macros before the \bibliography
%%% command.  Each of them MUST provide its own final punctuation,
%%% except for \shownote{}, \showDOI{}, and \showURL{}.  The latter two
%%% do not use final punctuation, in order to avoid confusing it with
%%% the Web address.
%%%
%%% To suppress output of a particular field, define its macro to expand
%%% to an empty string, or better, \unskip, like this:
%%%
%%% \newcommand{\showDOI}[1]{\unskip}   % LaTeX syntax
%%%
%%% \def \showDOI #1{\unskip}           % plain TeX syntax
%%%
%%% ====================================================================

\ifx \showCODEN    \undefined \def \showCODEN     #1{\unskip}     \fi
\ifx \showDOI      \undefined \def \showDOI       #1{#1}\fi
\ifx \showISBNx    \undefined \def \showISBNx     #1{\unskip}     \fi
\ifx \showISBNxiii \undefined \def \showISBNxiii  #1{\unskip}     \fi
\ifx \showISSN     \undefined \def \showISSN      #1{\unskip}     \fi
\ifx \showLCCN     \undefined \def \showLCCN      #1{\unskip}     \fi
\ifx \shownote     \undefined \def \shownote      #1{#1}          \fi
\ifx \showarticletitle \undefined \def \showarticletitle #1{#1}   \fi
\ifx \showURL      \undefined \def \showURL       {\relax}        \fi
% The following commands are used for tagged output and should be
% invisible to TeX
\providecommand\bibfield[2]{#2}
\providecommand\bibinfo[2]{#2}
\providecommand\natexlab[1]{#1}
\providecommand\showeprint[2][]{arXiv:#2}

\bibitem[Amini et~al\mbox{.}(2018)]%
        {amini2018evaluating}
\bibfield{author}{\bibinfo{person}{Fereshteh Amini}, \bibinfo{person}{Matthew Brehmer}, \bibinfo{person}{Gordon Bolduan}, \bibinfo{person}{Christina Elmer}, {and} \bibinfo{person}{Benjamin Wiederkehr}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Evaluating data-driven stories and storytelling tools}.
\newblock In \bibinfo{booktitle}{\emph{Data-driven storytelling}}. \bibinfo{publisher}{CRC Press}, \bibinfo{address}{Boca Raton, FL}, \bibinfo{pages}{249--286}.
\newblock
\showISBNx{9781138626593}
\urldef\tempurl%
\url{https://doi.org/10.1201/9781315281575-12}
\showDOI{\tempurl}


\bibitem[Bach et~al\mbox{.}(2016)]%
        {bashDynamicGraphComic}
\bibfield{author}{\bibinfo{person}{Benjamin Bach}, \bibinfo{person}{Natalie Kerracher}, \bibinfo{person}{Kyle~Wm. Hall}, \bibinfo{person}{Sheelagh Carpendale}, \bibinfo{person}{Jessie Kennedy}, {and} \bibinfo{person}{Nathalie Henry~Riche}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Telling Stories about Dynamic Networks with Graph Comics}. In \bibinfo{booktitle}{\emph{Proceedings of the 2016 CHI Conference on Human Factors in Computing Systems}} \emph{(\bibinfo{series}{CHI '16})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{3670–3682}.
\newblock
\showISBNx{9781450333627}
\urldef\tempurl%
\url{https://doi.org/10.1145/2858036.2858387}
\showDOI{\tempurl}


\bibitem[Bach et~al\mbox{.}(2014)]%
        {graphDiaries}
\bibfield{author}{\bibinfo{person}{Benjamin Bach}, \bibinfo{person}{Emmanuel Pietriga}, {and} \bibinfo{person}{Jean-Daniel Fekete}.} \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{GraphDiaries: Animated Transitions andTemporal Navigation for Dynamic Networks}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Visualization and Computer Graphics}} \bibinfo{volume}{20}, \bibinfo{number}{5} (\bibinfo{year}{2014}), \bibinfo{pages}{740--754}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1109/TVCG.2013.254}
\showDOI{\tempurl}


\bibitem[Bae et~al\mbox{.}(2024)]%
        {NetworkPhyAuthor}
\bibfield{author}{\bibinfo{person}{S.~Sandra Bae}, \bibinfo{person}{Takanori Fujiwara}, \bibinfo{person}{Anders Ynnerman}, \bibinfo{person}{Ellen Yi-Luen Do}, \bibinfo{person}{Michael~L. Rivera}, {and} \bibinfo{person}{Danielle~Albers Szafir}.} \bibinfo{year}{2024}\natexlab{}.
\newblock \showarticletitle{A Computational Design Pipeline to Fabricate Sensing Network Physicalizations}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Visualization and Computer Graphics}} \bibinfo{volume}{30}, \bibinfo{number}{1} (\bibinfo{year}{2024}), \bibinfo{pages}{913--923}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1109/TVCG.2023.3327198}
\showDOI{\tempurl}


\bibitem[Bae et~al\mbox{.}(2022)]%
        {SandraSurveyDataPhy}
\bibfield{author}{\bibinfo{person}{S.~Sandra Bae}, \bibinfo{person}{Clement Zheng}, \bibinfo{person}{Mary~Etta West}, \bibinfo{person}{Ellen Yi-Luen Do}, \bibinfo{person}{Samuel Huron}, {and} \bibinfo{person}{Danielle~Albers Szafir}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{Making Data Tangible: A Cross-disciplinary Design Space for Data Physicalization}. In \bibinfo{booktitle}{\emph{Proceedings of the 2022 CHI Conference on Human Factors in Computing Systems}} (New Orleans, LA, USA) \emph{(\bibinfo{series}{CHI '22})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, Article \bibinfo{articleno}{81}, \bibinfo{numpages}{18}~pages.
\newblock
\showISBNx{9781450391573}
\urldef\tempurl%
\url{https://doi.org/10.1145/3491102.3501939}
\showDOI{\tempurl}


\bibitem[Bounegru et~al\mbox{.}(2017)]%
        {NarratingNetworks}
\bibfield{author}{\bibinfo{person}{Liliana Bounegru}, \bibinfo{person}{Tommaso Venturini}, \bibinfo{person}{Jonathan Gray}, {and} \bibinfo{person}{Mathieu Jacomy}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Narrating Networks}.
\newblock \bibinfo{journal}{\emph{Digital Journalism}} \bibinfo{volume}{5}, \bibinfo{number}{6} (\bibinfo{year}{2017}), \bibinfo{pages}{699--730}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1080/21670811.2016.1186497}
\showDOI{\tempurl}


\bibitem[Brehmer and Kosara(2022)]%
        {FromJamtoRecital}
\bibfield{author}{\bibinfo{person}{Matthew Brehmer} {and} \bibinfo{person}{Robert Kosara}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{From Jam Session to Recital: Synchronous Communication and Collaboration Around Data in Organizations}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Visualization and Computer Graphics}} \bibinfo{volume}{28}, \bibinfo{number}{1} (\bibinfo{year}{2022}), \bibinfo{pages}{1139--1149}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1109/TVCG.2021.3114760}
\showDOI{\tempurl}


\bibitem[Cao et~al\mbox{.}(2024)]%
        {Elastica}
\bibfield{author}{\bibinfo{person}{Yining Cao}, \bibinfo{person}{Rubaiat~Habib Kazi}, \bibinfo{person}{Li-Yi Wei}, \bibinfo{person}{Deepali Aneja}, {and} \bibinfo{person}{Haijun Xia}.} \bibinfo{year}{2024}\natexlab{}.
\newblock \showarticletitle{Elastica: Adaptive Live Augmented Presentations with Elastic Mappings Across Modalities}. In \bibinfo{booktitle}{\emph{Proceedings of the CHI Conference on Human Factors in Computing Systems}} (Honolulu, HI, USA) \emph{(\bibinfo{series}{CHI '24})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, Article \bibinfo{articleno}{599}, \bibinfo{numpages}{19}~pages.
\newblock
\showISBNx{9798400703300}
\urldef\tempurl%
\url{https://doi.org/10.1145/3613904.3642725}
\showDOI{\tempurl}


\bibitem[Chen et~al\mbox{.}(2024)]%
        {CalliopeNet}
\bibfield{author}{\bibinfo{person}{Qing Chen}, \bibinfo{person}{Nan Chen}, \bibinfo{person}{Wei Shuai}, \bibinfo{person}{Guande Wu}, \bibinfo{person}{Zhe Xu}, \bibinfo{person}{Hanghang Tong}, {and} \bibinfo{person}{Nan Cao}.} \bibinfo{year}{2024}\natexlab{}.
\newblock \showarticletitle{Calliope-Net: Automatic Generation of Graph Data Facts via Annotated Node-Link Diagrams}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Visualization and Computer Graphics}} \bibinfo{volume}{30}, \bibinfo{number}{1} (\bibinfo{year}{2024}), \bibinfo{pages}{562--572}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1109/TVCG.2023.3326925}
\showDOI{\tempurl}


\bibitem[Cordeil et~al\mbox{.}(2020)]%
        {embodiedAxis}
\bibfield{author}{\bibinfo{person}{Maxime Cordeil}, \bibinfo{person}{Benjamin Bach}, \bibinfo{person}{Andrew Cunningham}, \bibinfo{person}{Bastian Montoya}, \bibinfo{person}{Ross~T. Smith}, \bibinfo{person}{Bruce~H. Thomas}, {and} \bibinfo{person}{Tim Dwyer}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{Embodied Axes: Tangible, Actuated Interaction for 3D Augmented Reality Data Spaces}. In \bibinfo{booktitle}{\emph{Proceedings of the 2020 CHI Conference on Human Factors in Computing Systems}} \emph{(\bibinfo{series}{CHI '20})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{1–12}.
\newblock
\showISBNx{9781450367080}
\urldef\tempurl%
\url{https://doi.org/10.1145/3313831.3376613}
\showDOI{\tempurl}


\bibitem[Dargue et~al\mbox{.}(2019)]%
        {dargue2019our}
\bibfield{author}{\bibinfo{person}{Nicole Dargue}, \bibinfo{person}{Naomi Sweller}, {and} \bibinfo{person}{Michael~P Jones}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{When our hands help us understand: A meta-analysis into the effects of gesture on comprehension}.
\newblock \bibinfo{journal}{\emph{Psychological Bulletin}} \bibinfo{volume}{145}, \bibinfo{number}{8} (\bibinfo{year}{2019}), \bibinfo{pages}{765}.
\newblock


\bibitem[Dimara et~al\mbox{.}(2022)]%
        {dimara2021unmet}
\bibfield{author}{\bibinfo{person}{Evanthia Dimara}, \bibinfo{person}{Harry Zhang}, \bibinfo{person}{Melanie Tory}, {and} \bibinfo{person}{Steven Franconeri}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{The Unmet Data Visualization Needs of Decision Makers Within Organizations}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Visualization and Computer Graphics}} \bibinfo{volume}{28}, \bibinfo{number}{12} (\bibinfo{year}{2022}), \bibinfo{pages}{4101--4112}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1109/TVCG.2021.3074023}
\showDOI{\tempurl}


\bibitem[Engle(2000)]%
        {engle2000toward}
\bibfield{author}{\bibinfo{person}{Randi~Alexandra Engle}.} \bibinfo{year}{2000}\natexlab{}.
\newblock \bibinfo{booktitle}{\emph{Toward a theory of multimodal communication: Combining speech, gestures, diagrams, and demonstrations in instructional explanations}}.
\newblock \bibinfo{publisher}{Stanford University}, \bibinfo{address}{Stanford, CA, USA}.
\newblock


\bibitem[Englmeier et~al\mbox{.}(2019)]%
        {sphere}
\bibfield{author}{\bibinfo{person}{David Englmeier}, \bibinfo{person}{Isabel Schönewald}, \bibinfo{person}{Andreas Butz}, {and} \bibinfo{person}{Tobias Höllerer}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Sphere in Hand: Exploring Tangible Interaction with Immersive Spherical Visualizations}. In \bibinfo{booktitle}{\emph{2019 IEEE Conference on Virtual Reality and 3D User Interfaces (VR)}}. \bibinfo{publisher}{IEEE}, \bibinfo{address}{Osaka, Japan}, \bibinfo{pages}{912--913}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1109/VR.2019.8797887}
\showDOI{\tempurl}


\bibitem[Ens et~al\mbox{.}(2021)]%
        {uplift}
\bibfield{author}{\bibinfo{person}{Barrett Ens}, \bibinfo{person}{Sarah Goodwin}, \bibinfo{person}{Arnaud Prouzeau}, \bibinfo{person}{Fraser Anderson}, \bibinfo{person}{Florence~Y. Wang}, \bibinfo{person}{Samuel Gratzl}, \bibinfo{person}{Zac Lucarelli}, \bibinfo{person}{Brendan Moyle}, \bibinfo{person}{Jim Smiley}, {and} \bibinfo{person}{Tim Dwyer}.} \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{Uplift: A Tangible and Immersive Tabletop System for Casual Collaborative Visual Analytics}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Visualization and Computer Graphics}} \bibinfo{volume}{27}, \bibinfo{number}{2} (\bibinfo{year}{2021}), \bibinfo{pages}{1193--1203}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1109/TVCG.2020.3030334}
\showDOI{\tempurl}


\bibitem[Femi-Gege et~al\mbox{.}(2024)]%
        {visConductor}
\bibfield{author}{\bibinfo{person}{Temiloluwa~Paul Femi-Gege}, \bibinfo{person}{Matthew Brehmer}, {and} \bibinfo{person}{Jian Zhao}.} \bibinfo{year}{2024}\natexlab{}.
\newblock \showarticletitle{VisConductor: Affect-Varying Widgets for Animated Data Storytelling in Gesture-Aware Augmented Video Presentation}.
\newblock \bibinfo{journal}{\emph{Proc. ACM Hum.-Comput. Interact.}} \bibinfo{volume}{8}, \bibinfo{number}{ISS}, Article \bibinfo{articleno}{531} (\bibinfo{date}{Oct.} \bibinfo{year}{2024}), \bibinfo{numpages}{22}~pages.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1145/3698131}
\showDOI{\tempurl}


\bibitem[Filipov et~al\mbox{.}(2023)]%
        {networkSurveyofSurvey}
\bibfield{author}{\bibinfo{person}{Velitchko Filipov}, \bibinfo{person}{Alessio Arleo}, {and} \bibinfo{person}{Silvia Miksch}.} \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{Are We There Yet? A Roadmap of Network Visualization from Surveys to Task Taxonomies}.
\newblock \bibinfo{journal}{\emph{Computer Graphics Forum}} \bibinfo{volume}{42}, \bibinfo{number}{6} (\bibinfo{year}{2023}), \bibinfo{pages}{e14794}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1111/cgf.14794}
\showDOI{\tempurl}


\bibitem[Fitzmaurice and Buxton(1997)]%
        {grappableUI}
\bibfield{author}{\bibinfo{person}{George~W. Fitzmaurice} {and} \bibinfo{person}{William Buxton}.} \bibinfo{year}{1997}\natexlab{}.
\newblock \showarticletitle{An empirical evaluation of graspable user interfaces: towards specialized, space-multiplexed input}. In \bibinfo{booktitle}{\emph{Proceedings of the ACM SIGCHI Conference on Human Factors in Computing Systems}} \emph{(\bibinfo{series}{CHI '97})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{43–50}.
\newblock
\showISBNx{0897918029}
\urldef\tempurl%
\url{https://doi.org/10.1145/258549.258578}
\showDOI{\tempurl}


\bibitem[Frisch et~al\mbox{.}(2009)]%
        {multitouchGraph}
\bibfield{author}{\bibinfo{person}{Mathias Frisch}, \bibinfo{person}{Jens Heydekorn}, {and} \bibinfo{person}{Raimund Dachselt}.} \bibinfo{year}{2009}\natexlab{}.
\newblock \showarticletitle{Investigating multi-touch and pen gestures for diagram editing on interactive surfaces}. In \bibinfo{booktitle}{\emph{Proceedings of the ACM International Conference on Interactive Tabletops and Surfaces}} \emph{(\bibinfo{series}{ITS '09})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{149–156}.
\newblock
\showISBNx{9781605587332}
\urldef\tempurl%
\url{https://doi.org/10.1145/1731903.1731933}
\showDOI{\tempurl}


\bibitem[Fujiwara et~al\mbox{.}(2018)]%
        {FUJIWARA2018213}
\bibfield{author}{\bibinfo{person}{Takanori Fujiwara}, \bibinfo{person}{Tarik Crnovrsanin}, {and} \bibinfo{person}{Kwan-Liu Ma}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Concise provenance of interactive network analysis}.
\newblock \bibinfo{journal}{\emph{Visual Informatics}} \bibinfo{volume}{2}, \bibinfo{number}{4} (\bibinfo{year}{2018}), \bibinfo{pages}{213--224}.
\newblock
\showISSN{2468-502X}
\urldef\tempurl%
\url{https://doi.org/10.1016/j.visinf.2018.12.002}
\showDOI{\tempurl}


\bibitem[Gong et~al\mbox{.}(2023)]%
        {affordanceBased}
\bibfield{author}{\bibinfo{person}{Weilun Gong}, \bibinfo{person}{Stephanie Santosa}, \bibinfo{person}{Tovi Grossman}, \bibinfo{person}{Michael Glueck}, \bibinfo{person}{Daniel Clarke}, {and} \bibinfo{person}{Frances Lai}.} \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{Affordance-Based and User-Defined Gestures for Spatial Tangible Interaction}. In \bibinfo{booktitle}{\emph{Proceedings of the 2023 ACM Designing Interactive Systems Conference}} \emph{(\bibinfo{series}{DIS '23})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{1500–1514}.
\newblock
\showISBNx{9781450398930}
\urldef\tempurl%
\url{https://doi.org/10.1145/3563657.3596032}
\showDOI{\tempurl}


\bibitem[{Google LLC}(2024)]%
        {googlemeet}
\bibfield{author}{\bibinfo{person}{{Google LLC}}.} \bibinfo{year}{2024}\natexlab{}.
\newblock \bibinfo{title}{Google Meet: Secure Video Meetings}.
\newblock \bibinfo{howpublished}{\url{https://meet.google.com}}.
\newblock
\newblock
\shownote{Accessed: 2024-11-29}.


\bibitem[Gyory et~al\mbox{.}(2023)]%
        {ARUCODesignSpace}
\bibfield{author}{\bibinfo{person}{Peter Gyory}, \bibinfo{person}{S.~Sandra Bae}, \bibinfo{person}{Ruhan Yang}, \bibinfo{person}{Ellen Yi-Luen Do}, {and} \bibinfo{person}{Clement Zheng}.} \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{Marking Material Interactions with Computer Vision}. In \bibinfo{booktitle}{\emph{Proceedings of the 2023 CHI Conference on Human Factors in Computing Systems}} \emph{(\bibinfo{series}{CHI '23})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, Article \bibinfo{articleno}{478}, \bibinfo{numpages}{17}~pages.
\newblock
\showISBNx{9781450394215}
\urldef\tempurl%
\url{https://doi.org/10.1145/3544548.3580643}
\showDOI{\tempurl}


\bibitem[Hall et~al\mbox{.}(2022)]%
        {Chironomia}
\bibfield{author}{\bibinfo{person}{Brian~D. Hall}, \bibinfo{person}{Lyn Bartram}, {and} \bibinfo{person}{Matthew Brehmer}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{Augmented Chironomia for Presenting Data to Remote Audiences}. In \bibinfo{booktitle}{\emph{Proceedings of the 35th Annual ACM Symposium on User Interface Software and Technology}} (Bend, OR, USA) \emph{(\bibinfo{series}{UIST '22})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, Article \bibinfo{articleno}{18}, \bibinfo{numpages}{14}~pages.
\newblock
\showISBNx{9781450393201}
\urldef\tempurl%
\url{https://doi.org/10.1145/3526113.3545614}
\showDOI{\tempurl}


\bibitem[He et~al\mbox{.}(2024)]%
        {DataCube}
\bibfield{author}{\bibinfo{person}{Shuqi He}, \bibinfo{person}{Haonan Yao}, \bibinfo{person}{Luyan Jiang}, \bibinfo{person}{Kaiwen Li}, \bibinfo{person}{Nan Xiang}, \bibinfo{person}{Yue Li}, \bibinfo{person}{Hai-Ning Liang}, {and} \bibinfo{person}{Lingyun Yu}.} \bibinfo{year}{2024}\natexlab{}.
\newblock \showarticletitle{Data Cubes in Hand: A Design Space of Tangible Cubes for Visualizing 3D Spatio-Temporal Data in Mixed Reality}. In \bibinfo{booktitle}{\emph{Proceedings of the CHI Conference on Human Factors in Computing Systems}} \emph{(\bibinfo{series}{CHI '24})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, Article \bibinfo{articleno}{209}, \bibinfo{numpages}{21}~pages.
\newblock
\showISBNx{9798400703300}
\urldef\tempurl%
\url{https://doi.org/10.1145/3613904.3642740}
\showDOI{\tempurl}


\bibitem[Hettiarachchi and Wigdor(2016)]%
        {AnnexingReality}
\bibfield{author}{\bibinfo{person}{Anuruddha Hettiarachchi} {and} \bibinfo{person}{Daniel Wigdor}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Annexing Reality: Enabling Opportunistic Use of Everyday Objects as Tangible Proxies in Augmented Reality}. In \bibinfo{booktitle}{\emph{Proceedings of the 2016 CHI Conference on Human Factors in Computing Systems}} (San Jose, California, USA) \emph{(\bibinfo{series}{CHI '16})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{1957–1967}.
\newblock
\showISBNx{9781450333627}
\urldef\tempurl%
\url{https://doi.org/10.1145/2858036.2858134}
\showDOI{\tempurl}


\bibitem[Ishii and Ullmer(1997)]%
        {TangibleBit}
\bibfield{author}{\bibinfo{person}{Hiroshi Ishii} {and} \bibinfo{person}{Brygg Ullmer}.} \bibinfo{year}{1997}\natexlab{}.
\newblock \showarticletitle{Tangible bits: towards seamless interfaces between people, bits and atoms}. In \bibinfo{booktitle}{\emph{Proceedings of the ACM SIGCHI Conference on Human Factors in Computing Systems}} \emph{(\bibinfo{series}{CHI '97})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{234–241}.
\newblock
\showISBNx{0897918029}
\urldef\tempurl%
\url{https://doi.org/10.1145/258549.258715}
\showDOI{\tempurl}


\bibitem[Jackson et~al\mbox{.}(2013)]%
        {cylinder}
\bibfield{author}{\bibinfo{person}{Bret Jackson}, \bibinfo{person}{Tung~Yuen Lau}, \bibinfo{person}{David Schroeder}, \bibinfo{person}{Kimani~C. Toussaint}, {and} \bibinfo{person}{Daniel~F. Keefe}.} \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{A Lightweight Tangible 3D Interface for Interactive Visualization of Thin Fiber Structures}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Visualization and Computer Graphics}} \bibinfo{volume}{19}, \bibinfo{number}{12} (\bibinfo{year}{2013}), \bibinfo{pages}{2802--2809}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1109/TVCG.2013.121}
\showDOI{\tempurl}


\bibitem[Jansen and Dragicevic(2013)]%
        {BeyondDesktop}
\bibfield{author}{\bibinfo{person}{Yvonne Jansen} {and} \bibinfo{person}{Pierre Dragicevic}.} \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{An Interaction Model for Visualizations Beyond The Desktop}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Visualization and Computer Graphics}} \bibinfo{volume}{19}, \bibinfo{number}{12} (\bibinfo{year}{2013}), \bibinfo{pages}{2396--2405}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1109/TVCG.2013.134}
\showDOI{\tempurl}


\bibitem[Kim et~al\mbox{.}(2025)]%
        {DGComics}
\bibfield{author}{\bibinfo{person}{Joohee Kim}, \bibinfo{person}{Hyunwook Lee}, \bibinfo{person}{Duc~M. Nguyen}, \bibinfo{person}{Minjeong Shin}, \bibinfo{person}{Bum~Chul Kwon}, \bibinfo{person}{Sungahn Ko}, {and} \bibinfo{person}{Niklas Elmqvist}.} \bibinfo{year}{2025}\natexlab{}.
\newblock \showarticletitle{DG Comics: Semi-Automatically Authoring Graph Comics for Dynamic Graphs}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Visualization and Computer Graphics}} \bibinfo{volume}{31}, \bibinfo{number}{1} (\bibinfo{year}{2025}), \bibinfo{pages}{973--983}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1109/TVCG.2024.3456340}
\showDOI{\tempurl}


\bibitem[Kim et~al\mbox{.}(2019)]%
        {kimDataToon}
\bibfield{author}{\bibinfo{person}{Nam~Wook Kim}, \bibinfo{person}{Nathalie Henry~Riche}, \bibinfo{person}{Benjamin Bach}, \bibinfo{person}{Guanpeng Xu}, \bibinfo{person}{Matthew Brehmer}, \bibinfo{person}{Ken Hinckley}, \bibinfo{person}{Michel Pahud}, \bibinfo{person}{Haijun Xia}, \bibinfo{person}{Michael~J. McGuffin}, {and} \bibinfo{person}{Hanspeter Pfister}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{DataToon: Drawing Dynamic Network Comics With Pen + Touch Interaction}. In \bibinfo{booktitle}{\emph{Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems}} (Glasgow, Scotland Uk) \emph{(\bibinfo{series}{CHI '19})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{1–12}.
\newblock
\showISBNx{9781450359702}
\urldef\tempurl%
\url{https://doi.org/10.1145/3290605.3300335}
\showDOI{\tempurl}


\bibitem[Kosara and Mackinlay(2013)]%
        {kosara2013storytelling}
\bibfield{author}{\bibinfo{person}{Robert Kosara} {and} \bibinfo{person}{Jock Mackinlay}.} \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{Storytelling: The Next Step for Visualization}.
\newblock \bibinfo{journal}{\emph{Computer}} \bibinfo{volume}{46}, \bibinfo{number}{5} (\bibinfo{year}{2013}), \bibinfo{pages}{44--50}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1109/MC.2013.36}
\showDOI{\tempurl}


\bibitem[Le~Goc et~al\mbox{.}(2019)]%
        {CompositeUsingWheeled}
\bibfield{author}{\bibinfo{person}{Mathieu Le~Goc}, \bibinfo{person}{Charles Perin}, \bibinfo{person}{Sean Follmer}, \bibinfo{person}{Jean-Daniel Fekete}, {and} \bibinfo{person}{Pierre Dragicevic}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Dynamic Composite Data Physicalization Using Wheeled Micro-Robots}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Visualization and Computer Graphics}} \bibinfo{volume}{25}, \bibinfo{number}{1} (\bibinfo{date}{Jan.} \bibinfo{year}{2019}), \bibinfo{pages}{737–747}.
\newblock
\showISSN{1077-2626}
\urldef\tempurl%
\url{https://doi.org/10.1109/TVCG.2018.2865159}
\showDOI{\tempurl}


\bibitem[Lee et~al\mbox{.}(2013)]%
        {LeeSketchStory}
\bibfield{author}{\bibinfo{person}{Bongshin Lee}, \bibinfo{person}{Rubaiat~Habib Kazi}, {and} \bibinfo{person}{Greg Smith}.} \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{SketchStory: Telling More Engaging Stories with Data through Freeform Sketching}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Visualization and Computer Graphics}} \bibinfo{volume}{19}, \bibinfo{number}{12} (\bibinfo{year}{2013}), \bibinfo{pages}{2416--2425}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1109/TVCG.2013.191}
\showDOI{\tempurl}


\bibitem[Lee et~al\mbox{.}(2006)]%
        {taskTaxonomyGraphBongshin}
\bibfield{author}{\bibinfo{person}{Bongshin Lee}, \bibinfo{person}{Catherine Plaisant}, \bibinfo{person}{Cynthia~Sims Parr}, \bibinfo{person}{Jean-Daniel Fekete}, {and} \bibinfo{person}{Nathalie Henry}.} \bibinfo{year}{2006}\natexlab{}.
\newblock \showarticletitle{Task taxonomy for graph visualization}. In \bibinfo{booktitle}{\emph{Proceedings of the 2006 AVI Workshop on BEyond Time and Errors: Novel Evaluation Methods for Information Visualization}} (Venice, Italy) \emph{(\bibinfo{series}{BELIV '06})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{1–5}.
\newblock
\showISBNx{1595935622}
\urldef\tempurl%
\url{https://doi.org/10.1145/1168149.1168168}
\showDOI{\tempurl}


\bibitem[Lefeuvre et~al\mbox{.}(2018)]%
        {bricks}
\bibfield{author}{\bibinfo{person}{Kevin Lefeuvre}, \bibinfo{person}{Soeren Totzauer}, \bibinfo{person}{Michael Storz}, \bibinfo{person}{Albrecht Kurze}, \bibinfo{person}{Andreas Bischof}, {and} \bibinfo{person}{Arne Berger}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Bricks, Blocks, Boxes, Cubes, and Dice: On the Role of Cubic Shapes for the Design of Tangible Interactive Devices}. In \bibinfo{booktitle}{\emph{Proceedings of the 2018 Designing Interactive Systems Conference}} \emph{(\bibinfo{series}{DIS '18})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{485–496}.
\newblock
\showISBNx{9781450351980}
\urldef\tempurl%
\url{https://doi.org/10.1145/3196709.3196768}
\showDOI{\tempurl}


\bibitem[Li et~al\mbox{.}(2024)]%
        {dataStorySurveyHaotian}
\bibfield{author}{\bibinfo{person}{Haotian Li}, \bibinfo{person}{Yun Wang}, {and} \bibinfo{person}{Huamin Qu}.} \bibinfo{year}{2024}\natexlab{}.
\newblock \showarticletitle{Where Are We So Far? Understanding Data Storytelling Tools from the Perspective of Human-AI Collaboration}. In \bibinfo{booktitle}{\emph{Proceedings of the CHI Conference on Human Factors in Computing Systems}} \emph{(\bibinfo{series}{CHI '24})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, Article \bibinfo{articleno}{845}, \bibinfo{numpages}{19}~pages.
\newblock
\showISBNx{9798400703300}
\urldef\tempurl%
\url{https://doi.org/10.1145/3613904.3642726}
\showDOI{\tempurl}


\bibitem[Li et~al\mbox{.}(2023)]%
        {networkNerratives}
\bibfield{author}{\bibinfo{person}{Wenchao Li}, \bibinfo{person}{Sarah Sch\"{o}ttler}, \bibinfo{person}{James Scott-Brown}, \bibinfo{person}{Yun Wang}, \bibinfo{person}{Siming Chen}, \bibinfo{person}{Huamin Qu}, {and} \bibinfo{person}{Benjamin Bach}.} \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{NetworkNarratives: Data Tours for Visual Network Exploration and Analysis}. In \bibinfo{booktitle}{\emph{Proceedings of the 2023 CHI Conference on Human Factors in Computing Systems}} (Hamburg, Germany) \emph{(\bibinfo{series}{CHI '23})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, Article \bibinfo{articleno}{172}, \bibinfo{numpages}{15}~pages.
\newblock
\showISBNx{9781450394215}
\urldef\tempurl%
\url{https://doi.org/10.1145/3544548.3581452}
\showDOI{\tempurl}


\bibitem[Liao et~al\mbox{.}(2022)]%
        {RealityTalk}
\bibfield{author}{\bibinfo{person}{Jian Liao}, \bibinfo{person}{Adnan Karim}, \bibinfo{person}{Shivesh~Singh Jadon}, \bibinfo{person}{Rubaiat~Habib Kazi}, {and} \bibinfo{person}{Ryo Suzuki}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{RealityTalk: Real-Time Speech-Driven Augmented Presentation for AR Live Storytelling}. In \bibinfo{booktitle}{\emph{Proceedings of the 35th Annual ACM Symposium on User Interface Software and Technology}} \emph{(\bibinfo{series}{UIST '22})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, Article \bibinfo{articleno}{17}, \bibinfo{numpages}{12}~pages.
\newblock
\showISBNx{9781450393201}
\urldef\tempurl%
\url{https://doi.org/10.1145/3526113.3545702}
\showDOI{\tempurl}


\bibitem[Lund(2007)]%
        {lund2007importance}
\bibfield{author}{\bibinfo{person}{Kristine Lund}.} \bibinfo{year}{2007}\natexlab{}.
\newblock \showarticletitle{The Importance of Gaze and Gesture in Interactive Multimodal Explanation}.
\newblock \bibinfo{journal}{\emph{Language Resources and Evaluation}}  \bibinfo{volume}{41} (\bibinfo{year}{2007}), \bibinfo{pages}{289--303}.
\newblock
\showISSN{1574-020X}
\urldef\tempurl%
\url{https://doi.org/10.1007/s10579-007-9048-2}
\showDOI{\tempurl}


\bibitem[Morris et~al\mbox{.}(2014)]%
        {primingTech}
\bibfield{author}{\bibinfo{person}{Meredith~Ringel Morris}, \bibinfo{person}{Andreea Danielescu}, \bibinfo{person}{Steven Drucker}, \bibinfo{person}{Danyel Fisher}, \bibinfo{person}{Bongshin Lee}, \bibinfo{person}{m.~c. schraefel}, {and} \bibinfo{person}{Jacob~O. Wobbrock}.} \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{Reducing legacy bias in gesture elicitation studies}.
\newblock \bibinfo{journal}{\emph{Interactions}} \bibinfo{volume}{21}, \bibinfo{number}{3} (\bibinfo{date}{may} \bibinfo{year}{2014}), \bibinfo{pages}{40–45}.
\newblock
\showISSN{1072-5520}
\urldef\tempurl%
\url{https://doi.org/10.1145/2591689}
\showDOI{\tempurl}


\bibitem[Newman(2018)]%
        {newman2018networks}
\bibfield{author}{\bibinfo{person}{Mark Newman}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \bibinfo{booktitle}{\emph{Networks}}.
\newblock \bibinfo{publisher}{Oxford University Press}, \bibinfo{address}{Oxford, UK}.
\newblock
\showISBNx{9780198805090}


\bibitem[Ojo and Heravi(2018)]%
        {PatternsinAwardWinning}
\bibfield{author}{\bibinfo{person}{Adegboyega Ojo} {and} \bibinfo{person}{Bahareh Heravi}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Patterns in Award Winning Data Storytelling}.
\newblock \bibinfo{journal}{\emph{Digital Journalism}} \bibinfo{volume}{6}, \bibinfo{number}{6} (\bibinfo{year}{2018}), \bibinfo{pages}{693--718}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1080/21670811.2017.1403291}
\showDOI{\tempurl}


\bibitem[Potts et~al\mbox{.}(2022)]%
        {TangibleTouch}
\bibfield{author}{\bibinfo{person}{Dominic Potts}, \bibinfo{person}{Martynas Dabravalskis}, {and} \bibinfo{person}{Steven Houben}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{TangibleTouch: A Toolkit for Designing Surface-based Gestures for Tangible Interfaces}. In \bibinfo{booktitle}{\emph{Proceedings of the Sixteenth International Conference on Tangible, Embedded, and Embodied Interaction}} \emph{(\bibinfo{series}{TEI '22})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, Article \bibinfo{articleno}{39}, \bibinfo{numpages}{14}~pages.
\newblock
\showISBNx{9781450391474}
\urldef\tempurl%
\url{https://doi.org/10.1145/3490149.3502263}
\showDOI{\tempurl}


\bibitem[Price et~al\mbox{.}(2003)]%
        {tangibelGoodEngagement}
\bibfield{author}{\bibinfo{person}{S Price}, \bibinfo{person}{Y Rogers}, \bibinfo{person}{M Scaife}, \bibinfo{person}{D Stanton}, {and} \bibinfo{person}{H Neale}.} \bibinfo{year}{2003}\natexlab{}.
\newblock \showarticletitle{Using 'tangibles' to promote novel forms of playful learning}.
\newblock \bibinfo{journal}{\emph{Interacting with Computers}} \bibinfo{volume}{15}, \bibinfo{number}{2} (\bibinfo{year}{2003}), \bibinfo{pages}{169--185}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1016/S0953-5438(03)00006-7}
\showDOI{\tempurl}


\bibitem[Riche et~al\mbox{.}(2018)]%
        {riche2018data}
\bibfield{author}{\bibinfo{person}{Nathalie~Henry Riche}, \bibinfo{person}{Christophe Hurter}, \bibinfo{person}{Nicholas Diakopoulos}, {and} \bibinfo{person}{Sheelagh Carpendale}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \bibinfo{booktitle}{\emph{Data-Driven Storytelling}}.
\newblock \bibinfo{publisher}{CRC Press}, \bibinfo{address}{Boca Raton, FL}.
\newblock
\showISBNx{9781138626593}
\urldef\tempurl%
\url{https://doi.org/10.1201/9781315281575}
\showDOI{\tempurl}


\bibitem[Romat et~al\mbox{.}(2021)]%
        {ExpressiveAuthoringNodeLink}
\bibfield{author}{\bibinfo{person}{Hugo Romat}, \bibinfo{person}{Caroline Appert}, {and} \bibinfo{person}{Emmanuel Pietriga}.} \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{Expressive Authoring of Node-Link Diagrams With Graphies}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Visualization and Computer Graphics}} \bibinfo{volume}{27}, \bibinfo{number}{4} (\bibinfo{year}{2021}), \bibinfo{pages}{2329--2340}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1109/TVCG.2019.2950932}
\showDOI{\tempurl}


\bibitem[Rosling(2007)]%
        {rosling2007best}
\bibfield{author}{\bibinfo{person}{Hans Rosling}.} \bibinfo{year}{2007}\natexlab{}.
\newblock \bibinfo{title}{The best stats you've ever seen}.
\newblock \bibinfo{howpublished}{\url{https://www.youtube.com/watch?v=hVimVzgtD6w}}.
\newblock


\bibitem[Rosling(2011)]%
        {rosling2011countries}
\bibfield{author}{\bibinfo{person}{Hans Rosling}.} \bibinfo{year}{2011}\natexlab{}.
\newblock \bibinfo{title}{Hans Rosling's 200 Countries, 200 Years, 4 Minutes}.
\newblock \bibinfo{howpublished}{\url{https://www.youtube.com/watch?v=jbkSRLYSojo}}.
\newblock


\bibitem[Rosling(2014)]%
        {rosling2014global}
\bibfield{author}{\bibinfo{person}{Hans Rosling}.} \bibinfo{year}{2014}\natexlab{}.
\newblock \bibinfo{title}{Global population growth, box by box}.
\newblock \bibinfo{howpublished}{\url{https://www.ted.com/talks/hans_rosling_global_population_growth_box_by_box}}.
\newblock


\bibitem[Rosling(2015)]%
        {rosling2015ignorant}
\bibfield{author}{\bibinfo{person}{Hans Rosling}.} \bibinfo{year}{2015}\natexlab{}.
\newblock \bibinfo{title}{How not to be ignorant about the world}.
\newblock \bibinfo{howpublished}{\url{https://www.youtube.com/watch?v=Sm5xF-UYgdg}}.
\newblock


\bibitem[Rosling(2016a)]%
        {rosling2016global}
\bibfield{author}{\bibinfo{person}{Hans Rosling}.} \bibinfo{year}{2016}\natexlab{a}.
\newblock \bibinfo{title}{Numbers are boring, people are interesting}.
\newblock \bibinfo{howpublished}{\url{https://www.youtube.com/watch?v=nh94kK05l-M&ab_channel=TEDxTalks}}.
\newblock


\bibitem[Rosling(2016b)]%
        {rosling2016world}
\bibfield{author}{\bibinfo{person}{Hans Rosling}.} \bibinfo{year}{2016}\natexlab{b}.
\newblock \bibinfo{title}{Why the world population won't exceed 11 billion}.
\newblock \bibinfo{howpublished}{\url{https://www.youtube.com/watch?v=2LyzBoHo5EI}}.
\newblock


\bibitem[Rufiange and McGuffin(2013)]%
        {DiffAni}
\bibfield{author}{\bibinfo{person}{Sébastien Rufiange} {and} \bibinfo{person}{Michael~J. McGuffin}.} \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{DiffAni: Visualizing Dynamic Graphs with a Hybrid of Difference Maps and Animation}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Visualization and Computer Graphics}} \bibinfo{volume}{19}, \bibinfo{number}{12} (\bibinfo{year}{2013}), \bibinfo{pages}{2556--2565}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1109/TVCG.2013.149}
\showDOI{\tempurl}


\bibitem[Saquib et~al\mbox{.}(2019)]%
        {BodyDrivenTalk}
\bibfield{author}{\bibinfo{person}{Nazmus Saquib}, \bibinfo{person}{Rubaiat~Habib Kazi}, \bibinfo{person}{Li-Yi Wei}, {and} \bibinfo{person}{Wilmot Li}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Interactive Body-Driven Graphics for Augmented Video Performance}. In \bibinfo{booktitle}{\emph{Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems}} \emph{(\bibinfo{series}{CHI '19})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{1–12}.
\newblock
\showISBNx{9781450359702}
\urldef\tempurl%
\url{https://doi.org/10.1145/3290605.3300852}
\showDOI{\tempurl}


\bibitem[Satriadi et~al\mbox{.}(2023)]%
        {activeProxyDash}
\bibfield{author}{\bibinfo{person}{Kadek~Ananta Satriadi}, \bibinfo{person}{Barrett Ens}, \bibinfo{person}{Sarah Goodwin}, {and} \bibinfo{person}{Tim Dwyer}.} \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{Active Proxy Dashboard: Binding Physical Referents and Abstract Data Representations in Situated Visualization through Tangible Interaction}. In \bibinfo{booktitle}{\emph{Extended Abstracts of the 2023 CHI Conference on Human Factors in Computing Systems}} \emph{(\bibinfo{series}{CHI EA '23})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, Article \bibinfo{articleno}{23}, \bibinfo{numpages}{7}~pages.
\newblock
\showISBNx{9781450394222}
\urldef\tempurl%
\url{https://doi.org/10.1145/3544549.3585797}
\showDOI{\tempurl}


\bibitem[Satriadi et~al\mbox{.}(2022)]%
        {tangibleGlobe}
\bibfield{author}{\bibinfo{person}{Kadek~Ananta Satriadi}, \bibinfo{person}{Jim Smiley}, \bibinfo{person}{Barrett Ens}, \bibinfo{person}{Maxime Cordeil}, \bibinfo{person}{Tobias Czauderna}, \bibinfo{person}{Benjamin Lee}, \bibinfo{person}{Ying Yang}, \bibinfo{person}{Tim Dwyer}, {and} \bibinfo{person}{Bernhard Jenny}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{Tangible Globes for Data Visualisation in Augmented Reality}. In \bibinfo{booktitle}{\emph{Proceedings of the 2022 CHI Conference on Human Factors in Computing Systems}} \emph{(\bibinfo{series}{CHI '22})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, Article \bibinfo{articleno}{505}, \bibinfo{numpages}{16}~pages.
\newblock
\showISBNx{9781450391573}
\urldef\tempurl%
\url{https://doi.org/10.1145/3491102.3517715}
\showDOI{\tempurl}


\bibitem[Segel and Heer(2010)]%
        {SegelNarrative}
\bibfield{author}{\bibinfo{person}{Edward Segel} {and} \bibinfo{person}{Jeffrey Heer}.} \bibinfo{year}{2010}\natexlab{}.
\newblock \showarticletitle{Narrative Visualization: Telling Stories with Data}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Visualization and Computer Graphics}} \bibinfo{volume}{16}, \bibinfo{number}{6} (\bibinfo{year}{2010}), \bibinfo{pages}{1139--1148}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1109/TVCG.2010.179}
\showDOI{\tempurl}


\bibitem[Seokmin~Kang and Black(2015)]%
        {CoordinationForPresentation}
\bibfield{author}{\bibinfo{person}{Barbara~Tversky Seokmin~Kang} {and} \bibinfo{person}{John~B. Black}.} \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{Coordinating Gesture, Word, and Diagram: Explanations for Experts and Novices}.
\newblock \bibinfo{journal}{\emph{Spatial Cognition \& Computation}} \bibinfo{volume}{15}, \bibinfo{number}{1} (\bibinfo{year}{2015}), \bibinfo{pages}{1--26}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1080/13875868.2014.958837}
\showDOI{\tempurl}


\bibitem[Shaer and Hornecker(2010)]%
        {TUItextbook}
\bibfield{author}{\bibinfo{person}{Orit Shaer} {and} \bibinfo{person}{Eva Hornecker}.} \bibinfo{year}{2010}\natexlab{}.
\newblock \showarticletitle{Tangible User Interfaces: Past, Present, and Future Directions}.
\newblock \bibinfo{journal}{\emph{Found. Trends Hum.-Comput. Interact.}} \bibinfo{volume}{3}, \bibinfo{number}{1–2} (\bibinfo{date}{jan} \bibinfo{year}{2010}), \bibinfo{pages}{1–137}.
\newblock
\showISSN{1551-3955}
\urldef\tempurl%
\url{https://doi.org/10.1561/1100000026}
\showDOI{\tempurl}


\bibitem[Spritzer et~al\mbox{.}(2015)]%
        {SpritzerStaticNet}
\bibfield{author}{\bibinfo{person}{Andre~Suslik Spritzer}, \bibinfo{person}{Jeremy Boy}, \bibinfo{person}{Pierre Dragicevic}, \bibinfo{person}{Jean-Daniel Fekete}, {and} \bibinfo{person}{Carla~Maria Dal Sasso~Freitas}.} \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{Towards a smooth design process for static communicative node-link diagrams}.
\newblock \bibinfo{journal}{\emph{Computer Graphics Forum}} \bibinfo{volume}{34}, \bibinfo{number}{3} (\bibinfo{year}{2015}), \bibinfo{pages}{461--470}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1111/cgf.12658}
\showDOI{\tempurl}


\bibitem[Srinivasan and Brehmer(2023)]%
        {srinivasancombining}
\bibfield{author}{\bibinfo{person}{Arjun Srinivasan} {and} \bibinfo{person}{Matthew Brehmer}.} \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{Combining Voice and Gesture for Presenting Data to Remote Audiences}. In \bibinfo{booktitle}{\emph{IEEE VIS 2023 Workshop on Multimodal Experiences for Remote Communication Around Data Online, MERCADO'23}}. \bibinfo{publisher}{IEEE Educational Activities Department}, \bibinfo{address}{Melbourne, Australia}, \bibinfo{pages}{1--2}.
\newblock
\urldef\tempurl%
\url{arjun010.github.io/static/papers/mm-presentationmercado23.pdf}
\showURL{%
\tempurl}


\bibitem[Srinivasan and Stasko(2018)]%
        {orko}
\bibfield{author}{\bibinfo{person}{Arjun Srinivasan} {and} \bibinfo{person}{John Stasko}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Orko: Facilitating Multimodal Interaction for Visual Exploration and Analysis of Networks}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Visualization and Computer Graphics}} \bibinfo{volume}{24}, \bibinfo{number}{1} (\bibinfo{year}{2018}), \bibinfo{pages}{511--521}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1109/TVCG.2017.2745219}
\showDOI{\tempurl}


\bibitem[Streeck(1993)]%
        {GestureAsCommunication}
\bibfield{author}{\bibinfo{person}{Jürgen Streeck}.} \bibinfo{year}{1993}\natexlab{}.
\newblock \showarticletitle{Gesture as communication I: Its coordination with gaze and speech}.
\newblock \bibinfo{journal}{\emph{Communication Monographs}} \bibinfo{volume}{60}, \bibinfo{number}{4} (\bibinfo{year}{1993}), \bibinfo{pages}{275--299}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1080/03637759309376314}
\showDOI{\tempurl}


\bibitem[Suzuki et~al\mbox{.}(2019)]%
        {shapebot}
\bibfield{author}{\bibinfo{person}{Ryo Suzuki}, \bibinfo{person}{Clement Zheng}, \bibinfo{person}{Yasuaki Kakehi}, \bibinfo{person}{Tom Yeh}, \bibinfo{person}{Ellen Yi-Luen Do}, \bibinfo{person}{Mark~D. Gross}, {and} \bibinfo{person}{Daniel Leithinger}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{ShapeBots: Shape-changing Swarm Robots}. In \bibinfo{booktitle}{\emph{Proceedings of the 32nd Annual ACM Symposium on User Interface Software and Technology}} (New Orleans, LA, USA) \emph{(\bibinfo{series}{UIST '19})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{493–505}.
\newblock
\showISBNx{9781450368162}
\urldef\tempurl%
\url{https://doi.org/10.1145/3332165.3347911}
\showDOI{\tempurl}


\bibitem[Taher et~al\mbox{.}(2015)]%
        {physicallyDynamicBar}
\bibfield{author}{\bibinfo{person}{Faisal Taher}, \bibinfo{person}{John Hardy}, \bibinfo{person}{Abhijit Karnik}, \bibinfo{person}{Christian Weichel}, \bibinfo{person}{Yvonne Jansen}, \bibinfo{person}{Kasper Hornb\ae{}k}, {and} \bibinfo{person}{Jason Alexander}.} \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{Exploring Interactions with Physically Dynamic Bar Charts}. In \bibinfo{booktitle}{\emph{Proceedings of the 33rd Annual ACM Conference on Human Factors in Computing Systems}} (Seoul, Republic of Korea) \emph{(\bibinfo{series}{CHI '15})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{3237–3246}.
\newblock
\showISBNx{9781450331456}
\urldef\tempurl%
\url{https://doi.org/10.1145/2702123.2702604}
\showDOI{\tempurl}


\bibitem[Tong et~al\mbox{.}(2023)]%
        {PaperVis}
\bibfield{author}{\bibinfo{person}{Wai Tong}, \bibinfo{person}{Chen Zhu-Tian}, \bibinfo{person}{Meng Xia}, \bibinfo{person}{Leo Yu-Ho Lo}, \bibinfo{person}{Linping Yuan}, \bibinfo{person}{Benjamin Bach}, {and} \bibinfo{person}{Huamin Qu}.} \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{Exploring Interactions with Printed Data Visualizations in Augmented Reality}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Visualization and Computer Graphics}} \bibinfo{volume}{29}, \bibinfo{number}{1} (\bibinfo{year}{2023}), \bibinfo{pages}{418--428}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1109/TVCG.2022.3209386}
\showDOI{\tempurl}


\bibitem[Ullmer and Ishii(2000)]%
        {IshiiTUI}
\bibfield{author}{\bibinfo{person}{B. Ullmer} {and} \bibinfo{person}{H. Ishii}.} \bibinfo{year}{2000}\natexlab{}.
\newblock \showarticletitle{Emerging frameworks for tangible user interfaces}.
\newblock \bibinfo{journal}{\emph{IBM Systems Journal}} \bibinfo{volume}{39}, \bibinfo{number}{3.4} (\bibinfo{year}{2000}), \bibinfo{pages}{915--931}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1147/sj.393.0915}
\showDOI{\tempurl}


\bibitem[Veldhuis et~al\mbox{.}(2020)]%
        {Coda}
\bibfield{author}{\bibinfo{person}{Annemiek Veldhuis}, \bibinfo{person}{Rong-Hao Liang}, {and} \bibinfo{person}{Tilde Bekker}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{CoDa: Collaborative Data Interpretation Through an Interactive Tangible Scatterplot}. In \bibinfo{booktitle}{\emph{Proceedings of the Fourteenth International Conference on Tangible, Embedded, and Embodied Interaction}} (Sydney NSW, Australia) \emph{(\bibinfo{series}{TEI '20})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{323–336}.
\newblock
\showISBNx{9781450361071}
\urldef\tempurl%
\url{https://doi.org/10.1145/3374920.3374934}
\showDOI{\tempurl}


\bibitem[{Xmind Ltd.}(2014)]%
        {xmind}
\bibfield{author}{\bibinfo{person}{{Xmind Ltd.}}} \bibinfo{year}{2014}\natexlab{}.
\newblock \bibinfo{title}{Xmind: A Full-Featured Mind Mapping and Brainstorming Tool}.
\newblock \bibinfo{howpublished}{\url{https://xmind.app}}.
\newblock
\newblock
\shownote{Version 8 Update 3, Accessed: 2024-09-11}.


\bibitem[Zhang et~al\mbox{.}(2024)]%
        {stick}
\bibfield{author}{\bibinfo{person}{Yaying Zhang}, \bibinfo{person}{Rongkai Shi}, {and} \bibinfo{person}{Hai-Ning Liang}.} \bibinfo{year}{2024}\natexlab{}.
\newblock \showarticletitle{Designing Stick-Based Extended Reality Controllers: A Participatory Approach}. In \bibinfo{booktitle}{\emph{Extended Abstracts of the 2024 CHI Conference on Human Factors in Computing Systems}} \emph{(\bibinfo{series}{CHI EA '24})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, Article \bibinfo{articleno}{103}, \bibinfo{numpages}{6}~pages.
\newblock
\showISBNx{9798400703317}
\urldef\tempurl%
\url{https://doi.org/10.1145/3613905.3650925}
\showDOI{\tempurl}


\bibitem[Zhao and Elmqvist(2022)]%
        {dataTV}
\bibfield{author}{\bibinfo{person}{Zhenpeng Zhao} {and} \bibinfo{person}{Niklas Elmqvist}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \bibinfo{title}{DataTV: Streaming Data Videos for Storytelling}.
\newblock
\newblock
\showeprint[arxiv]{2210.08175}~[cs.HC]
\urldef\tempurl%
\url{https://arxiv.org/abs/2210.08175}
\showURL{%
\tempurl}


\bibitem[{Zoom Video Communications, Inc.}(2024)]%
        {zoom}
\bibfield{author}{\bibinfo{person}{{Zoom Video Communications, Inc.}}} \bibinfo{year}{2024}\natexlab{}.
\newblock \bibinfo{title}{Zoom: Video Conferencing, Web Conferencing, Webinars, Screen Sharing}.
\newblock \bibinfo{howpublished}{\url{https://zoom.us}}.
\newblock
\newblock
\shownote{Version 5.15.2, Accessed: 2024-11-29}.


\end{thebibliography}

